Better Together: Online Probabilistic Clique Change Detection in 3D Landmark-Based Maps

Many modern simultaneous localization and mapping (SLAM) techniques rely on sparse landmark-based maps due to their real-time performance. However, these techniques frequently assert that these landmarks are fixed in position over time, known as the static-world assumption. This is rarely, if ever, the case in most real-world environments. Even worse, over long deployments, robots are bound to observe traditionally static landmarks change, for example when an autonomous vehicle encounters a construction zone. This work addresses this challenge, accounting for changes in complex three-dimensional environments with the creation of a probabilistic filter that operates on the features that give rise to landmarks. To accomplish this, landmarks are clustered into cliques and a filter is developed to estimate their persistence jointly among observations of the landmarks in a clique. This filter uses estimated spatial-temporal priors of geometric objects, allowing for dynamic and semi-static objects to be removed from a formally static map. The proposed algorithm is validated in a 3D simulated environment.

==> priors.tex <==
The work here hinges on knowing a prior distribution for the clique we are observing. 
However, as of yet, nothing has been presented to explain how this might be done. 
As in \cite{Rosen}, we admit the design of a variety of possible survival time priors $p_{T_\tau}(\cdot)$. 
However, dissenting from \cite{Rosen}, we believe that individual point are very unlikely to have enough information to accurately estimate its lifetime. Instead, we note that the lifetime of a point is likely highly correlated with the object it is resting on.
For example, a building is likely not to change for a very long time horizon, however, a car in a parking lot is likely to have a much shorter lifetime.

This motivates a class based prior as a simple yet effective approach to providing distribution over the lifetime of any given object in the environment, utilizing modern object detection networks such as \cite{YOLOv3,MaskRCNN} to correctly label features which lie within a instance when projected into the camera frame.
Adopting the exponential distribution previously mentioned as our prior for all objects is in line with normal survival analysis and makes generation of these priors straightforward, needing only a mean survival time to correctly parameterize the distribution.

A example procedure to generate mean survival times is as follows.
Using a set of collections spaced out over time, for each selection, we extract all instance detections from each timestep using a object detection network such as \cite{MaskRCNN}. 
Then, we iterate over each timestep within a sequence, using the mean depth measurement of the instance projected onto the image plane within the segmentation mask of the image, allowing us to use the pose of the robot to project out the point into 3D.
Using a approach motivated by \cite{MonoTracking}, at each timestep we have a number of proposal points which we integrate into the set of active tracks by performing the Hungarian algorithm over a set of tracks which integrate new measurements using a Kalman Filter.

This optimization uses the Manhalinobis distance of the 3d Kalman Filter to a proposal as the cost metric between tracks and proposals in 3D, with some upper cost to Birth on a proposal being poorly matched with all active tracks and creating a new track and a cost to lost for a track having no match in the proposals to go into a Lost state.
A track in the Lost state has a set number of iterations for retracking before being pulled out of the set of active tracks. 
This gives us a set of class labeled trajectories for objects observed along a trajectory of a robotic system.

One can then perform a similar matching between trajectory sequences at different times to find which objects have moved and which remain $\epsilon$ close to their initial position over a timeframe of collected data.
The cumulative matching over a dataset produces a collection of survival times, allowing one to take the mean survival time for a class and parameterize a prior for all features lying on that object.
